GeoSaddle: Geometry-Guided Saddle Networks for Periodic Ion Migration

Ion migration mechanisms govern ionic conductivity in solid electrolytes and battery electrodes, yet nudged elastic band (NEB) calculations require prescribed endpoints and an initial path, precluding the discovery of multi-step and concerted mechanisms with unknown intermediates. Here, we present GeoSaddle, which uses periodic geometric accessibility and channel directions to initialize local saddle searches on a potential energy surface (PES). Verified saddle-minimum connections supply relaxed product states for subsequent searches, and periodic occupancy matching assembles events into migration networks beyond a single endpoint pair. Using a foundation potential (FP), GeoSaddle required 12.7% of the model evaluations of an ellipsoidal PES-grid control on ten long, curved events. On 100 LiTraj paths, GeoSaddle recovered 92 paths with a 38.9% lower mean path root-mean-square deviation than bond-valence site energy guesses (0.120 vs. 0.196 $\mathring{\mathrm{A}}$) and 28% fewer subsequent FP NEB steps. GeoSaddle also reconstructed periodic vacancy, split-interstitial and knock-out relays in LiTi$_2$(PO$_4$)$_3$, Li$_{1+x}$Al$_x$Ti$_{2-x}$(PO$_4$)$_3$ (LATP) and Li$_4$P$_2$S$_6$, with quenched ab initio molecular dynamics states in LATP matching GeoSaddle network branches. In Li$_{10}$GeP$_2$S$_{12}$, three-Li and four-Li periodic relays preserved connectivity under full-ion density functional theory refinement, with peaks of 0.346 and 0.116 eV above their shared initial state. In pyrochlore Li$_{2-x}$La$_{(1+x)/3}$Nb$_2$O$_6$F, sublattice exploration resolved a six-step, three-Li relay with a 0.218 eV full-ion FP NEB peak and isolated the barrier reduction from local fluoride relaxation. Requiring only energies and forces, open-source GeoSaddle provides a general route from a host structure to verified, periodic migration networks.

==> xr_main.tex <==


